There are More Fish in the Sea: Automated Vulnerability Repair via Binary Templates

As software vulnerabilities increase in both volume and complexity, vendors often struggle to repair them promptly. Automated vulnerability repair has emerged as a promising solution to reduce the burden of manual debugging and fixing activities. However, existing techniques exclusively focus on repairing the vulnerabilities at the source code level, which has various limitations. For example, they are not applicable to those (e.g., users or security analysts) who do not have access to the source code. Consequently, this restricts the practical application of these techniques, especially in cases where vendors are unable to provide timely patches. In this paper, we aim to address the above limitations by performing vulnerability repair at binary code level, and accordingly propose a template-based automated vulnerability repair approach for Java binaries. Built on top of the literature, we collect fix templates from both existing template-based automated program repair approaches and vulnerability-specific analyses, which are then implemented for the Java binaries. Our systematic application of these templates effectively mitigates vulnerabilities: experiments on the Vul4J dataset demonstrate that TemVUR successfully repairs 11 vulnerabilities, marking a notable 57.1% improvement over current repair techniques. Moreover, TemVUR securely fixes 66.7% more vulnerabilities compared to leading techniques (15 vs. 9), underscoring its effectiveness in mitigating the risks posed by these vulnerabilities. To assess the generalizability of TemVUR, we curate the ManyVuls4J dataset, which goes beyond Vul4J to encompass a wider diversity of vulnerabilities. With 30% more vulnerabilities than its predecessor (increasing from 79 to 103). The evaluation on ManyVuls4J reaffirms TemVUR's effectiveness and generalizability across a diverse set of real-world vulnerabilities.

==> figures/repair_cases.tex <==

\begin{figure}[!t]
  \centering
  % \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{|p{25.625em}|}
    % \begin{tabular}{|c|}
    \hline
{\bf Statement-level repair from Chart-12}:
\\ \myminted{\textcolor{diffgray}{// Oracle Patch}}
\\ \myminted{\textcolor{diffred}{-  \colorbox{yellow}{this.dataset = dataset;}}}
\\ \myminted{\textcolor{diffgreen}{+  \colorbox{yellow}{setDataset(dataset);}}}
\\ \myminted{\textcolor{diffgray}{// Patch generated by GAMMA}}
\\ \myminted{\textcolor{diffred}{-  this.dataset = dataset;}}
\\ \myminted{\textcolor{diffgreen}{+  this.data = dataset;}}
\\\hline

{\bf Expression-level repair from Closure-123}:
\\ \myminted{\textcolor{diffgray}{// Oracle Patch}}
\\ \myminted{\textcolor{diffred}{- Context rhsContext =\colorbox{yellow}{Context.OTHER;}}}
\\ \myminted{\textcolor{diffgreen}{+ Context rhsContext =\colorbox{yellow}{getContextForNoInOperator(context);}}}
\\ \myminted{\textcolor{diffgray}{// Patch generated by GAMMA}}
\\ \myminted{\textcolor{diffred}{- Context rhsContext = Context.OTHER;}}
\\ \myminted{\textcolor{diffgreen}{+ Context rhsContext = Context.STATEMENT;}}
\\ \myminted{\textcolor{diffgray}{// Patch generated by Rap-Gen}}
\\ \myminted{\textcolor{diffred}{- Context rhsContext = Context.OTHER;}}
\\ \myminted{\textcolor{diffgreen}{+ ContextFactory rhsContext = getContext(context, false);}}
\\\hline

{\bf Token-level repair from Chart-24}:
\\ \myminted{\textcolor{diffgray}{// Oracle Patch}}
\\ \myminted{\textcolor{diffred}{-   int g = (int) ((\colorbox{yellow}{value} - this.lowerBound) / }}
\\ \myminted{\textcolor{diffred}{\quad\quad\quad 
(this.upperBound - this.lowerBound) * 255.0);}}
\\ \myminted{\textcolor{diffgreen}{+   int g = (int) ((\colorbox{yellow}{v} - this.lowerBound) /}}
\\ \myminted{\textcolor{diffgreen}{\quad\quad\quad 
 (this.upperBound - this.lowerBound) * 255.0);}}
\\ \myminted{\textcolor{diffgray}{// Patch generated by Rap-Gen}}
\\ \myminted{\textcolor{diffred}{-   int g = (int) ((value - this.lowerBound) / }}
\\ \myminted{\textcolor{diffred}{\quad\quad\quad 
 (this.upperBound - this.lowerBound) * 255.0);}}
\\ \myminted{\textcolor{diffgreen}{+   value = Math.min(v, this.lowerBound);}}
    \\
    \hline
    \end{tabular}%
    % }
  \caption{Program repair at different granularities.}
  \label{fig:repair_example}%
\end{figure}

==> figures/repair_cases_back.tex <==


\begin{figure}[!t]
  \centering
  \caption{Program Repair at different granularities}
  % \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{|p{25.625em}|}
    % \begin{tabular}{||}
    \hline
{\bf Statement-level repair from Chart-12}:
\begin{minted}[frame=none,
               linenos=none,
               numbersep=0pt,
               fontsize=\small,
               xleftmargin=0em,
               escapeinside=||
               ]{diff}
// Oracle Patch
|\textcolor{diffred}{-  \colorbox{yellow}{this.dataset = dataset;}}| 
|\textcolor{diffgreen}{+  \colorbox{yellow}{setDataset(dataset);}}| 
// Patch generated by GAMMA
-   this.dataset = dataset;
+   this.data = dataset;
\end{minted}
\\
    \hline
% {\bf Expression-level repair from Closure-104}:
% \begin{minted}[frame=none,
%                linenos=none,
%                numbersep=0pt,
%                fontsize=\small,
%                xleftmargin=0em,
%                ]{diff}         
% // Oracle Patch      
% -   if (result != null) {              
% +   if (!result.isNoType()) {     
%         return result;     
% // Patch generated by GAMMA
% -   if (result != null) {              
% +   if (result == null) {     
%         return result;    
% // Patch generated by Rap-Gen             
% -   if (result != null) {              
% +   if (that.isSubtype(result)) {     
%         return result;      
% \end{minted}

{\bf Expression-level repair from Closure-123}:
% \begin{minted}[frame=none,
%                linenos=none,
%                numbersep=0pt,
%                fontsize=\small,
%                xleftmargin=0em,
%                escapeinside=||
%                ]{diff}         
% // Oracle Patch      
% -  Context rhsContext = Context.OTHER;       
% +  Context rhsContext = getContextForNoInOperator(context); 
% // Patch generated by GAMMA
% -  Context rhsContext = Context.OTHER;          
% +  Context rhsContext = Context.STATEMENT;
% // Patch generated by Rap-Gen             
% -  Context rhsContext = Context.OTHER;          
% +  ContextFactory rhsContext = getContext(context, false);  
% \end{minted}

\begin{minted}[frame=none,
               linenos=none,
               numbersep=0pt,
               fontsize=\small,
               xleftmargin=0em,
               escapeinside=||
               ]{diff}         
// Oracle Patch      
|\textcolor{diffred}{- Context rhsContext =\colorbox{yellow}{Context.OTHER;}}| 
|\textcolor{diffgreen}{+ Context rhsContext =\colorbox{yellow}{getContextForNoInOperator(context);}}| 
// Patch generated by GAMMA
- Context rhsContext = Context.OTHER;          
+ Context rhsContext = Context.STATEMENT;
// Patch generated by Rap-Gen             
- Context rhsContext = Context.OTHER; 
+ ContextFactory rhsContext = getContext(context, false);  
\end{minted}

\\
    \hline

{\bf Token-level repair from Chart-24}:
\begin{minted}[frame=none,
               linenos=None,
               numbersep=0pt,
               fontsize=\small,
               xleftmargin=0em,
               escapeinside=||
               ]{diff}          
// Oracle Patch   
|\textcolor{diffred}{-   int g = (int) ((\colorbox{yellow}{value} - this.lowerBound) / }|
        |\textcolor{diffred}{(this.upperBound - this.lowerBound) * 255.0);}|
|\textcolor{diffgreen}{+   int g = (int) ((\colorbox{yellow}{v} - this.lowerBound) /}|
        |\textcolor{diffgreen}{(this.upperBound - this.lowerBound) * 255.0);}|
// Patch generated by Rap-Gen
-   int g = (int) ((value - this.lowerBound) / 
        |\textcolor{diffred}{(this.upperBound - this.lowerBound) * 255.0);}|
+   value = Math.min(v, this.lowerBound);
\end{minted}


% \vspace{-6mm}
    \\
    \hline
    \end{tabular}%
    % }
  \label{fig:repair_example}%
\end{figure}

==> figures/vul4j_31.tex <==
(@\textcolor{codegray}{// Developer-written patch}@)
+ import org.apache.struts2.StrutsException;
...
 } else {
- if (LOG.isWarnEnabled()) {
- ...
- return cleanActionName;
+ throw new StrutsException("Action [" + rawActionName + "] does not match allowed action names pattern [" + allowedActionNames + "]!");

(@\textcolor{codegray}{// \toolname's patch}@)
...
 } else {
+ return "";
...


==> figures/vul4j_59.tex <==
  currentAccessPermission = new AccessPermission(dicPermissions);
+ currentAccessPermission.setReadOnly();
  setCurrentAccessPermission(currentAccessPermission);

==> listings/NullChecker.tex <==
(@\phantom{x}\hspace{0ex}{\bf T2.1:}\hspace{2ex} \textcolor{codegreen}{+}@)  if (exp != null) {   
(@\phantom{x}\hspace{15ex}@) ...exp...; ......
(@\phantom{x}\hspace{6.7ex} \textcolor{codegreen}{+}@)  }
(@\phantom{x}{\bf T2.2:}\hspace{2ex} \textcolor{codegreen}{+}@)  if (exp == null) return DEFAULT_VALUE;  
(@\phantom{x}\hspace{11ex}@) ...exp...;
(@\phantom{x}{\bf T2.3:}\hspace{2ex} \textcolor{codegreen}{+}@)  if (exp == null) exp = exp1;  
(@\phantom{x}\hspace{11ex}@) ...exp...;
(@\phantom{x}{\bf T2.4:}\hspace{2ex} \textcolor{codegreen}{+}@)  if (exp == null) continue;  
(@\phantom{x}\hspace{11ex}@) ...exp...;
(@\phantom{x}{\bf T2.5:}\hspace{2ex} \textcolor{codegreen}{+}@)  if (exp == null)
(@\phantom{x}\hspace{6.7ex} \textcolor{codegreen}{+}\hspace{6ex}@)throw new IllegalArgumentException(...);  
(@\phantom{x}\hspace{11ex}@) ...exp...;




==> tables/D4J_performance.tex <==
% \begin{table}[!t]
%   \centering
%   \caption{Performances of different approaches on the Defects4J v1.2 and v2.0 dataset(in number of correct repairs). \bo{Should we report a lower performance?}}
%   \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{l|cc}
%     \toprule
%     \textbf{Approach}  & {\textbf{Defects4J v1.2}}& {\textbf{Defects4J v2.0}} \\
%     \hline
%     $\text{PraPR}^*\dagger$ & 41    & - \\
%     $\text{TBar}^*$  & 68    & 8 \\
%     CoCoNuT & 43    & - \\
%     RewardRepair & 44    & 43 \\
%     CURE  & 55    & - \\
%     Recoder & 64    & 11 \\
%     SelfAPR & 65    & 45 \\
%     RAP-Gen & 72    & 53 \\
%     AlphaRepair & 74    & 36 \\
%     GAMMA & 82    & 45 \\
%     \hline
%     \toolname   & \bf{99} & \bf{74} \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \label{tab:d4jn_res}%
%   \begin{tablenotes}
% 	\small
%         \item $^*$ PraPR and TBar are template-based tools. 
% 		\item $^\dagger$ PraPR is evaluated with the results of Ochiai fault localization\cite{wong2016survey}. 
%         \item ``-'' indicates data unavailability.
% 	\end{tablenotes}
% \end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{The performance of different approaches on the Defects4J v1.2 and v2.0 dataset (in number of correct repairs).}
    \begin{tabular}{ccccc}
    \toprule
\multirow{2}{*}{Tool} & \multicolumn{2}{c}{Perfect FL} & \multicolumn{2}{c}{Spectrum-based FL}\\ 
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
  & v1.2 & v2.0 & v1.2 & v2.0 \\ 
    \midrule
    $\text{PraPR}^\dagger$ & -     & -     & 41    & - \\
    $\text{TBar}^\dagger$  & 68    & 8     & 43    & - \\
    CoCoNuT & 43    & -     & -     & - \\
    RewardRepair & 44    & 43    & 27    & 24 \\
    CURE  & 55    & 19     & 38     & 11 \\
    SelfAPR & 63    & 45    & 39    & 28 \\
    Recoder & 65    & 19    & 49    & 9 \\
    Repilot & 66    & 50    & 47    & 30 \\
    RAP-Gen & 72    & 53    & 48    & 26 \\
    AlphaRepair & 74    & 36    & 50    & 20 \\
    GAMMA & 82    & 45    & 47     & 20 \\
    \midrule
    \toolname & \bf{92}    & \bf{59}    & \bf{56}    & \bf{31} \\
    \bottomrule
    \end{tabular}%
    \label{tab:d4j_res}%
  \begin{tablenotes}
	\small
        \item $^\dagger$ PraPR and TBar are template-based tools. 
        \item ``-'' indicates data unavailability.
	\end{tablenotes}
\end{table}%


==> tables/Vul4J_Info.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  % \centering
  \caption{The projects included in the Vul4J dataset}
  \resizebox{0.97\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
        \multicolumn{1}{l}{Project } & \multicolumn{1}{l}{Vuls} & \multicolumn{1}{l}{kLOC} & \multicolumn{1}{l}{Tests} & \multicolumn{1}{l}{CWEs} \\
    \midrule
    apache/struts   &  10   &   359 &  1697  &  6\\
    apache/commons-compress &   4   &    48  &   927   & 2\\
    jenkinsci/jenkins &   3  &  275   &  518    &  2\\
    spring-projects/spring-framework &   3   &  684    &  2189    &  2\\
    spring-projects/spring-security &  3  &  198  &  513  & 3\\
    apache/camel &   2  &  925    &   5222   & 1\\
    apache/commons-fileupload &  2    &  6  &  70  & 2\\
    apache/commons-imaging &  2    &  42  &   562   & 1 \\
    apache/cxf  &  2   &   737   &  89    &  2 \\
    apache/pdfbox & 2    &   145    &  359     & 1 \\
    apache/sling &   2    &   507    &   25    &  2\\
    cloudfoundry/uaa &  2    &   182   &  2669    & 2\\
    FasterXML/jackson-dataformat-xml &  2     &   9   &   140   & 2\\
    inversoft/prime-jwt &  2    &   2    &   33    & 1 \\
    OpenRefine/OpenRefine & 2     &  144     &   516    & 2 \\
    Others (mean) &   1   &    121   &   567    & 1 \\
    \midrule 
    Average &  1.55   &   169    &   705    & 1.31 \\
    \bottomrule
    \end{tabular}%
    }
    
  \label{tab:vul4jInfo}%
\end{table}%


==> tables/Vul4J_performance_FL.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  % \centering
  \caption{Comparison with state-of-the-art APR and AVR techniques under spectrum-based fault localization on Vul4J dataset}
  \resizebox{0.97\linewidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
          & \multicolumn{1}{l}{Plausible } & \multicolumn{1}{l}{Security-Fixing} & \multicolumn{1}{l}{Correct} & \multicolumn{1}{l}{\%Correct} \\
    \midrule
    ARJA  &  5  &  5   &   3 & 60.0 \\
    Cardumen &   6   &   3   &   2   & 33.3 \\
    GenProg-A &  4   &   4   &   2   & 50.0 \\
    jGenProg &   5   &   4   &   2   & 40.0 \\
    jKali   &  5  &  4 &  2  & 40.0 \\
    jMutRepair &   3  &  1    &   1   & 33.3\\
    Kali-A &   5   &  4  &  3 & 60.0 \\
    RSRepair-A &   5   &  4   &   3  & 60.0 \\
    TBar  &   7  &   5   &   3   & 42.9 \\
    PraPR &  6   &   5    &   4    & 66.7 \\
    GAMMA &   6    &   4    &    4   & 66.7 \\
    SeqTrans &   2   &   2   &   2   & \bf{100.0} \\
    VulRepair-J &   6    &  5    &  5    & 83.3 \\
    VulRepairE-J &  7  &   6    &   5    & 71.4 \\
    \midrule
    \toolname &   \bf{9}   & \bf{9}  &  \bf{7}  & 77.8 \\
    \bottomrule
    \end{tabular}%
    }
    % {\scriptsize "\%Correct" is the ratio of correct patches over plausible patches.}
  \label{tab:vul4j_FL}%
\end{table}%


==> tables/Vul4J_performance_PF.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'

\begin{table}[htbp]
  % \centering
  \caption{Comparison with state-of-the-art APR and AVR techniques under perfect fault localization on Vul4J dataset}
  \resizebox{0.97\linewidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
          & \multicolumn{1}{l}{Plausible } & \multicolumn{1}{l}{Security-Fixing} & \multicolumn{1}{l}{Correct} & \multicolumn{1}{l}{\%Correct$^{*}$} \\
    \midrule
    ARJA  & 8     & 8     & 5     & 62.5 \\
    Cardumen & 8     & 3     & 2     & 25.0 \\
    GenProg-A & 6     & 6     & 2     & 33.3 \\
    jGenProg & 7     & 4     & 2     & 28.6 \\
    jKali & 8     & 5     & 3     & 37.5 \\
    jMutRepair & 5     & 2     & 1     & 20.0 \\
    Kali-A & 7     & 6     & 3     & 42.9 \\
    RSRepair-A & 7     & 7     & 5     & 71.4 \\
    TBar  & 11    & 7     & 5     &  45.5 \\
    PraPR & 9     &  8     &   6    &  66.7 \\
    GAMMA &  10  &   7    &   6    &  60.0 \\
    SeqTrans & 2     & 2     & 2     &  \bf{100.0} \\
    VulRepair-J &  12     &  8     &  6     & 50.0 \\
    VulRepairE-J &  12     &   9    &  7     &  58.3 \\
    \midrule
    \toolname &  \bf{16}    &  \bf{15}     & \bf{11}    & 68.8 \\
    \bottomrule
    \end{tabular}%
    }
    {\footnotesize
    \begin{flushleft} $^{*}$ \%Correct is the ratio of correct patches over plausible patches.
    \end{flushleft}
    }
  \label{tab:vul4j_PF}%
\end{table}%


==> tables/vul_perf_types.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{\toolname's effectiveness on the Top-10 most frequent CWEs.}
  \resizebox{0.98\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    CWE Type & Name  & PP  & Proportion \\
    \midrule
     CWE-119 & \makecell[c]{Improper Restriction of Operations \\within the Bounds of a Memory Buffer} & 29.9 & 92/308 \\
     CWE-125 & Out-of-bounds Read & 25.0 & 28/112 \\
     CWE-20 & Improper Input Validation & 26.7 & 28/105 \\
     CWE-264 & Permissions, Privileges, and Access Controls & 46.0 & 23/50 \\
     CWE-476 & NULL Pointer Dereference & 40.9 & 18/44 \\
     CWE-200 & \makecell[c]{Exposure of Sensitive Information to \\an Unauthorized Actor} & 37.2 & 16/43 \\
     CWE-416 & Use After Free & 35.7 & 15/42 \\
     CWE-190 & Integer Overflow or Wraparound & 34.2 & 15/38 \\
     CWE-787 & Out-of-bounds Write & 34.4 & 11/32 \\
     CWE-399 & Resource Management Errors & 41.9 & 11/31 \\ \hline
     Total    &  & 31.9& 257/805\\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:vul_perf_type}%
\end{table}%

